Shared Cross-Modal Trajectory Prediction for Autonomous Driving

Predicting future trajectories of traffic agents in highly interactive environments is an essential and challenging problem for the safe operation of autonomous driving systems. On the basis of the fact that self-driving vehicles are equipped with various types of sensors (e.g., LiDAR scanner, RGB camera, radar, etc.), we propose a Cross-Modal Embedding framework that aims to benefit from the use of multiple input modalities. At training time, our model learns to embed a set of complementary features in a shared latent space by jointly optimizing the objective functions across different types of input data. At test time, a single input modality (e.g., LiDAR data) is required to generate predictions from the input perspective (i.e., in the LiDAR space), while taking advantages from the model trained with multiple sensor modalities. An extensive evaluation is conducted to show the efficacy of the proposed framework using two benchmark driving datasets.

==> notations.tex <==
\section{Preliminaries}

Given a scenario with the motion data $\mathcal{X}=\{{X}^i|\forall i\in \{1,...,K\}\}$ of $K$ traffic agents, we split ${X}^i$ into a past trajectory $\mathbf{r}^i = \{r^i_{t}|\forall t\in\{1,...,\tau\}\}$ for the first $\tau$ observation time steps and a future trajectory $\mathbf{x}^i = \{x^i_{t}|\forall t\in\{1,...,\delta\}\}$ for the next $\delta$ time steps. Assuming that a corresponding visual sequence $\mathcal{I} = \{I_{t}|\forall t\in\{1,...,\tau\}\}$ is available during $\tau$ observation time steps, we compute the optical flow $\mathcal{O} = \{O_{1:2}, O_{2:3}, ..., O_{\tau-1:\tau}\}$ and segmentation map $S$. Given $\{\mathcal{O},S\}$ and $\mathcal{X}$, our goal is to predict a future trajectory $\mathbf{x}^k$ of the target agent $k$. To achieve this, we build a feature extraction module upon graph neural networks in order to learn social behaviors $\mathbf{y}^k$ of the target agent $k$ toward all other traffic agents (\textit{e.g.}, pedestrians, vehicles, etc.) as well as surrounding road structures. Then, the encoder $q(\mathbf{z}|\mathbf{x}^k,\mathbf{y}^k)$ embeds $\mathbf{y}^k$ into the latent space. The following decoder $p(\mathbf{x}^k|\mathbf{z},\mathbf{y}^k)$ finds the future locations ${\mathbf{x}^k}$ of the target agent $k$ using the latent sample $\mathbf{z}$. Note that we do not distinguish the notations of different input modalities unless otherwise mentioned. \\

% \noindent \textbf{Message Passing Neural Networks (MPNN)} Message Passing Neural Networks (MPNN) framework~\cite{gilmer2017neural} operates on undirected graphs $G$ with node features $x_v$ and edge features $e_{vw}$. The forward pass has two phases, a message passing phase and a readout phase. The message passing phase runs for $T$ time steps and is defined in terms of message functions $M_t$
% and vertex update functions $U_t$. During the message passing phase, hidden states $\mathbf{h}^t_v$ at each node in the graph are updated based on messages $\mathbf{m}^{t+1}_v$ according to
% \begin{align}
%     \mathbf{m}_v^{t+1} &= \sum_{w \in N(v)} M_t \left( \mathbf{h}_v^t, \mathbf{h}_w^t, e_{vw} \right) \\
%     \mathbf{h}_v^{t+1} &= U_t \left( \mathbf{h}_v^t, \mathbf{m}_v^{t+1} \right), \label{eqn:1}
% \end{align}
% where in the sum, $N(v)$ denotes the neighbors of $v$ in graph $G$. The readout phase computes a feature vector for the whole graph using some readout function $R$ according to 
% \begin{equation}
%     \hat{y} = R \left( \{ \mathbf{h}_v^T | v \in G \} \right).
% \end{equation}
% The message functions $M_t$, vertex update functions $U_t$, and readout function $R$ are all learned differentiable functions. $R$ operates on the set of node states and must be invariant to
% permutations of the node states in order for the MPNN to be invariant to graph isomorphism.

%Let's define a graph $G = ({H},F)$, where $H\in\mathbb{R}^{K\times d_V}$, $H=\{\mathbf{h}^i|\forall i\in\{1,...,K\}\}$ is a node feature matrix representing $K$ node embeddings of size $d_V$. $F\in\mathbb{R}^{K\times d_E}$ is an external feature matrix $F=\{\mathbf{f}^i|\forall i\in\{1,...,K\}\}$, where each entity represents outside influence on each node in the graph. Following the general message passing phases~\cite{gilmer2017neural}, we construct a graph neural network (GNN) architecture for agent-specific social behavior modeling:
%\begin{equation}
%\begin{tabular}{rcl}
%    $\mathbf{m}^k_{(l)}$&$=$&$Agg\left(M(\mathbf{h}^i_{(l-1)},\mathbf{h}^j_{(l-1)},\mathbf{h}^k_{(l-1)},\mathbf{f}^i,\mathbf{f}^j)\right)$\\
%    &&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~$\forall i,j\in\{1,...,K\}$\\    $\mathbf{h}^k_{(l)}$&$=$&$U(\mathbf{h}^k_{(l-1)},\mathbf{m}^k_{(l)})$,
%\end{tabular}\label{eqn:1}
%\end{equation}
%where $M$ is a message generation function, $Agg$ is an aggregation function (\textit{e.g.}, sum and mean), and $U$ is a node feature update function. During the message passing phase, the relation between two nodes $i$ and $j$ is encoded with respect to the target node features $\mathbf{h}^k_{(l-1)}$ by considering their external influences $\{\mathbf{f}^i,\mathbf{f}^j\}$ through the function $M$. Then, the features of the target node $\mathbf{h}^k_{(l)}$ in the graph are updated using the messages $\mathbf{m}^k_{(l)}$. After $L$ updates, we convert the final node features $\mathbf{h}^k_{(L)}$ into social behavior features for the target agent $k$ in a given scenario. %Note that we do not explicitly define edge features in the graph. Instead, the relations between every two nodes are generated and propagated to update the node features. 

%\noindent 
%\textbf{Input Modalities}
%Any set of sensory data can be used as input to the proposed framework. For demonstration, however, we use two exemplary data types that are easily accessible from currently developing autonomous vehicles: (i) \textit{LiDAR data} provide 3D scanning of the surrounding environment. Using 3D point clouds, we project every single point onto the ground plane in top-down view and predict trajectories of traffic agents in the LiDAR-captured world coordinates. (ii) \textit{RGB images} captured from a frontal-facing camera provide rich and dense representations. We predict the trajectories from the egocentric perspective in the image space, following the literature~\cite{Yagi_2018_CVPR,yao2018egocentric}. Unlike their relative trajectories, our predicted trajectories are the absolute locations with respect to the first observation frame, eliminating the effect of the future motion of ego-vehicle. The data preparation is detailed in the supplementary material.

%Note that the input modalities are not limited to these two types but also include stereo images, depth, radar, GPS, and many others equipped in autonomous vehicles, which can provide visual or locational information. The method from other types is almost the same as that from LiDAR data and RGB images.

% \subsection{Dataset Preprocessing}
% , which is grounded into a certain reference frame (\textit{i.e.}, the first frame of each trajectory segment).


%\noindent
%\textbf{Problem Formulation} Given a scenario with the motion data $\mathcal{X}=\{{X}^i|\forall i\in \{1,...,K\}\}$ of $K$ traffic agents, we split ${X}^i$ into a past trajectory $\mathbf{r}^i = \{r^i_{t}|\forall t\in\{1,...,\tau\}\}$ for the first $\tau$ observation time steps and a future trajectory $\mathbf{x}^i = \{x^i_{t}|\forall t\in\{1,...,\delta\}\}$ for the next $\delta$ time steps. Assuming that a corresponding visual sequence $\mathcal{I} = \{I_{t}|\forall t\in\{1,...,\tau\}\}$ is available during $\tau$ observation time steps, we compute the optical flow $\mathcal{O} = \{O_{1}, O_{2}, ..., O_{\tau-1}\}$ and segmentation map $S$. Given $\{\mathcal{O},S\}$ and $\mathcal{X}$, our goal is to predict a future trajectory $\mathbf{x}^k$ of the target agent $k$. To achieve this, we build a feature extraction module upon graph neural networks in order to learn social behaviors $\mathbf{y}^k$ of the target agent $k$ toward all other traffic agents (\textit{e.g.}, pedestrians, vehicles, etc.) as well as surrounding road structures. Then, the encoder $q(\mathbf{z}|\mathbf{x}^k,\mathbf{y}^k)$ embeds $\mathbf{y}^k$ into the latent space. The following decoder $p(\mathbf{x}^k|\mathbf{z},\mathbf{y}^k)$ finds the future locations ${\mathbf{x}^k}$ of the target agent $k$ using the latent sample $\mathbf{z}$. Note that we do not distinguish the notations of different input modalities unless otherwise mentioned. 


